General Support-Effective Decomposition for Multi-Directional 3D Printing

We present a method for fabricating general models with multi-directional 3D printing systems by printing different model regions along with different directions. The core of our method is a support-effective volume decomposition algorithm that minimizes the area of the regions with large overhangs. A beam-guided searching algorithm with manufacturing constraints determines the optimal volume decomposition, which is represented by a sequence of clipping planes. While current approaches require manually assembling separate components into a final model, our algorithm allows for directly printing the final model in a single pass. It can also be applied to models with loops and handles. A supplementary algorithm generates special supporting structures for models where supporting structures for large overhangs cannot be eliminated. We verify the effectiveness of our method using two hardware systems: a Cartesian-motion based system and an angular-motion based system. A variety of 3D models have been successfully fabricated on these systems.

==> algorithm.tex <==
\section{Volume Decopmosition}
 




\subsection{Greedy search approach}
\label{sec:greedy}

\begin{figure}[t]
\centering
\includegraphics[width=0.95 \linewidth]{fig/figManufacturable.jpg}
\caption{A description of the manufacturable decomposition.} 
\label{figManufacturable}
\end{figure}

Unlike existing decomposition methods adopting manual assembly to avoid introducing collision problem into the printing process, we aim to find an integrated solution that models can be decomposed and printed in a closed loop. Tedious manual assembly becomes unnecessary by orienting to different printing directions automatically with the help of a multi-directional printing system. To obtain the desired decomposition result, we need to solve a constrained search problem over an infinite space: if any collision between the already printed object and printing system occurs, the printing will crash even could be harmful to the printing system; otherwise, we call it \emph{manufacturable} (see Fig. \ref{figManufacturable}). 

\begin{figure}[t]
\includegraphics[width=0.95 \linewidth]{fig/figPeelModel.png}
\caption{A 2D illustration of the greedy decomposition approach. From left to right: (1) The input tree model is first cut by the purple line and then the green line. (2)-(4) the fabrication sequence is the reversed sequence of cuttings. } 
\label{figGreedyApproach}
\end{figure}

Assume that we use a complete plane $\pi$ to clip a model $\mathcal{M}$, the region $\mathcal{R}_+$ defined by the positive side of $\pi$ is manufacturable if we print the object(s) $\mathcal{M}_i \in \mathcal{R}_+(\pi)$ in the direction perpendicular to $\pi_+$ at a time. According to this observation, we propose a greedy search approach which uses planar cuttings to peel the input model successively until the resulting decomposition satisfies our demands. 

The multi-directional printing systems need a sequence of printing the parts after decomposition, a feasible sequence $S$ of printing should satisfy collision-free requirement otherwise the whole printing procedure may fail. In this case, the problem of planning $S$ can be simplified with the help of the natural convexity of planar clipping. The greedy search results in a forward decomposition sequence and the fabrication sequence can be easily obtained by reversing the forward decomposition sequence, which means that $S$ can be obtained by reversing the order of clippings (see Fig. \ref{figGreedyApproach}).

The proposed greedy algorithm tends to successively use planes to cut meshes from the input mesh until a objective function is unchanged, following these three steps:

\begin{enumerate}
    \item Uniformly generate a set of candidate planes $\Pi=\{\pi\}$ for cutting the current mesh $\mathcal{M}$.
    \item Evaluate the objective function $f_g(\mathcal{R}_+\cap \mathcal{M}, n_{\pi_i})$ for each candidate plane $\pi_i$.
    \item Clip $\mathcal{M}$ by using the plane $\pi_o = \arg\min f_g(\cdot)$.
    \item Let $\mathcal{M}=\mathcal{M}-\mathcal{R}_+\cap \mathcal{M}$ and $M+=\mathcal{R}_+\cap \mathcal{M}$ and go back to Step 1. 
\end{enumerate}

In this context, 
we define an objective function $f_g(\cdot)$ to minimize the usage of support structures over the search space. A natural setting for $f_g$ is putting the area of risky faces into consideration. Given a printing direction $\textbf{n}_{\pi_i}$ of a base plane $\pi_i$, any risky face $F_i \in \mathcal{F}_{risky} \subseteq \mathcal{F}_i$ of $\mathcal{M}_i$ can have the following function to evaluate its area of risky:

\begin{equation}
    r(F_i,\pi_i) = e(F_i, \pi_i) \cdot area(F_i) \cdot \cos\langle \textbf{n}_{\pi_i}, \textbf{n}_{F_i}\rangle 
\end{equation}

Then the risky area of a mesh $\mathcal{M}_i$ which is printed in the direction of the normal direction of the base plane $\pi_i$ can be obtained by:

\begin{equation}
    R(\mathcal{M}_i, \pi_i) = \sum_{F_j\in\mathcal{F}_i} r(F_j, \pi_i)
\end{equation}

We define an objective function $f_g$ for greedy search approach and the best-first cutting plane can be obtained as:

\begin{equation}
\begin{split}
\arg \max_{\pi_{i}} f_g(\mathcal{M}_g, \pi_i) = &R( \mathcal{M}_g, \pi_z) - (R(\mathcal{M}_g^p,\pi_i) \\
& +R(\mathcal{M}_g^n,\pi_z)) \\
s.t. \quad  \mathcal{M}_g & = \mathcal{M}_g^p \cup \mathcal{M}_g^n \\
\pi_{i} & = \mathcal{M}_g^p \cap \mathcal{M}_g^n \\
\pi_z & = (0,0,1)
\end{split}
\end{equation}
with $\mathcal{M}_g^p$ and $\mathcal{M}_g^n$ being the positive and negative sub-parts clipped from $\mathcal{M}_g$ by $\pi_{k,l}$ respectively.



The greedy objective has no control over the printability of decomposed results. For example, thin parts generated by planar clipping are unsuitable for 3D printing if the thickness is smaller than the nozzle's resolution. Moreover, an arbitrary planar clipping may generate floating regions on the negative side of a plane. These floating components need additional support structures and regions on the positive side of plane will be printed on the top of regions only supported by support structures, where the stability problem may occur. Therefore, we add two hard-constraints to the search framework to prevent these problems from happening as follows.

\begin{itemize}
    \item \textit{Thin part constraint:} The clipped regions have no point whose tangent plane is near parallel (say, the dot product of two unit normal vectors should be smaller than $0.9$) to the clipping plane and the distance is smaller than the nozzle's resolution. 
    \item \textit{Floating constraint:} The clipping plane can have multiple cross-sections, but the regions on the negative side of clipping plane can only have one connected component.
\end{itemize}

\vspace{5pt}








    
    








The greedy search algorithm works well for most 3D models, and it turns out an excellent performance on the speed of computation. Unfortunately, for some models with complicated topology, it often produces sub-optimal results. A common sense for greedy algorithms is that they are easily stuck by local minima, especially in the case that the search space is computation intractable. Meanwhile, the support-free requirement is stringent and the algorithm may easily fail if the models are having a complicated structure of topology.

As the difficulty of our problem, finding a global optimization method with constraints is impossible. We opt to propose a new solution using beam-guided search strategy to improve the quality of volume decomposition.



\subsection{Beam-guided search}

As the problem statement mentioned, our goal is to minimize the usage of support structures employing clipping an original model into several regions, each of which can be fabricated with fewer support structures or even without support structures. Instead of maximizing the decreased risky area of each clipping, we can also define a global objective function to describe our goal as:

\begin{equation}
    f_{global}(M) = \sum_{(\mathcal{M}_i, \pi_i)\in M} R(\mathcal{M}_i, \pi_i)
    \label{eq:globalFunc}
\end{equation}

The problem of finding an optimal decomposition of a globally minimal value of $f_{global}$ is non-trivial by exhaustively exploring the huge search space. Instead of directly using $f_{global}$ to explore, we opt to split the global search problem into a set of sub-problems by manufacturable heuristics and apply an efficient beam search algorithm to evaluate the decomposition from a different aspect of view to find the solutions. Finally, we use $f_{global}$ function to sort the results and users can easily select one of the most promising results accordingly. Based on the manufacturable analysis, we have the following criteria (i.e., manufacturable heuristics) for our support-effective multi-directional 3D printing:

\begin{itemize}
    \item {\makebox[2.6cm]{\textit{Criterion 1 (C1):}\hfill} All above regions are self-supported.}
    \item {\makebox[2.6cm]{\textit{Criterion 2 (C2):}\hfill}The working platform is below the clipping plane.}
    \item {\makebox[2.6cm]{\textit{Criterion 3 (C3):}\hfill}In case C1 cannot be satisfied, we try to keep as many as possible satisfied results and meanwhile minimizing the area of risky faces in the rest results (optionally).}
    \item {\makebox[2.6cm]{\textit{Criterion 4 (C4):}\hfill} Above region(s) is as large as possible (optionally).}
\end{itemize}

It is not easy to combine all the above four criteria in a comprehensive formula as they are sometimes controversial. For instance, a clipping of maximal volume might be useless if it was self-supported before. Or if we want to clip a region with a large amount of risky faces, its volume might not be compact or large. In our paper, we propose a new approach to solve the multi-objective optimization problem. We design a beam-guided search algorithm that integrates all above four criteria into a unified framework and use it to guide the search towards a non-local optimal solution evaluated by $f_{global}$.

\vspace{5pt}\noindent\textbf{Max risky area descent:} 
Having the goal of decreasing the area of risky faces in mind, we define a max risky area descent metric. This metric is concluded from criteria C1, C2 and C3; we define a function to help evaluate the quality of a decomposition.

\begin{equation}
    f_{local}^{area}(M) = \sum_{(\mathcal{M}_i,\pi_i)\in M} [ R(\mathcal{M}_i, \pi_z) - R(\mathcal{M}_i, \pi_i)]
    \label{eq:localFunc2}
\end{equation}

The most challenging part is how to integrate both strict criterion C1 and uncertain criterion C3 into one search process. Beam search \cite{Lowerre1976} is an efficient search technique which has been widely used in improving the results of the best-first greedy search, and it uses breadth-first strategy to build a search tree while exploring the search space by expanding a set of most promising nodes instead of only the best node in each level. It has been successfully used in a variety of areas especially in geometric configuration search tasks for 3D printing such as \cite{luo2012chopper,Chen2015dapper}. Instead of distinguishing too close results in the phase of selecting them from a set of evaluated results, we use beam search technique to relax C1 to C3 so the beam is full of different stage of the relaxation from C1 to C3. The relaxation procedure is modeled as a progressive relaxation, which integrates C4 to sample the middle stages progressively, as follows.

\vspace{5pt} \noindent \textbf{Progressive relaxation}: The fabrication process is the reverse process of decomposition, it is evident that if each clipped volume is small, the number of decomposition will be increased, which in turn influences the efficiency of fabrication as the number of rotations increases. Though we prefer to have a completely support-free result during each clipping, it may be very inefficient if the support-free regions are very small or even in-existent. To solve this problem in a unified way, we integrate C4 into our search algorithm and relax the C1 to have some choices which are not completely self-supported progressively. The function $f_{vol}$ determines the threshold $\epsilon$ of the area of risky faces according to the expected number of clippings $\Theta$ provided by users, note that $\Theta$ is not a hard-constraint and the algorithm may complete before reaching $\Theta$ clippings. The algorithm will progressively increase $\epsilon$ to allow more results with area of risky faces lower than $\epsilon$ and then put the element with maximal $f_{local}^{area}$ into the beam until the beam is fully occupied as expected.

\begin{equation}
    f_{vol}(\mathcal{M}_i) = 1 - \frac{\Theta \cdot V_{BBox}(\mathcal{M}_i, \pi_i)}{V(\mathcal{M})}
    \label{eq:Relaxation}
\end{equation}

\noindent where $V_{BBox}$ is the axis aligned bounding box of $\mathcal{M}_i$ with an axis aligned to $\pi_i$. \chenming{Try minimal bounding box with an axis aligned to $\pi_i$ later}

\vspace{5pt}



\begin{algorithm}[t]
\caption{\texttt{Beam-guided Search}}\label{algBeamGuidedSearch}

\LinesNumbered

\KwIn{Input mesh $\mathcal{M}$.}
\KwOut{A set of decomposed meshes $M$.}

\STATE Build a set of uniformly sampled candidate planes $\Pi$.

\While{no more solution found}{

\STATE $newResults \leftarrow \emptyset$

\For{each plane $\pi \in \Pi$}{
    \For{each res $\in$ currentResults}{
        \If{$\pi$ is intersecting with $res.\mathcal{M}$}
        {
            \STATE $newResults$ += $f_{local}^{area}(res.M,\pi)$
        }
    }
}

\STATE $Results \leftarrow\emptyset$



\While{$|Results| \neq b$}{
    \STATE $eps \leftarrow 0$
    
    \For{each $res$ $\in$ $sorted(newResults)$}{
        \STATE $\mathcal{M}^p, \mathcal{M}^n \leftarrow Clip(res.\mathcal{M}, res.\pi)$.

        \If{$f_{vol}(\mathcal{M}^p, \pi) \leq 0$ \rm \textbf{and} $ R(\mathcal{M}_{-1}, \pi_{-1}) \leq eps$}{
            \STATE $res.M$ += $\mathcal{M}_p$
            
            \STATE $res.\mathcal{M}$ = $\mathcal{M}-\mathcal{M}_n$ 
            
            \STATE $Results$ += $res$
        }
    }
    \STATE $eps += 1.0$
}
}

\For{each $res$ $\in$ $Results$}{

    \STATE $res.M$ += $res.\mathcal{M}$

}

\STATE Return $[\argmaxl_{res\in Results} f_{global}(res.M)].M$


\end{algorithm}


\vspace{5pt}\noindent \textbf{Beam-guided search:} Different from the traditional usage of a beam search algorithm that keeps the most $b$ promising results, our beam-guided search algorithm starts from an empty beam and $\epsilon=0$, then our algorithm adopts the progressive relaxation rule to fill in the beam with $b$ results and start next round of searching, which integrates all four criteria of support-effective multi-directional 3D printing together in a unified search framework. The expansion of different beam can be fused if a more promising $f_{local}^{area}$ can be achieved. This advantage helps the algorithm avoid local solutions and become more efficient towards an optimal result.

We describe the proposed algorithm in Alg. \ref{algBeamGuidedSearch}, and the experimental results verify the effectiveness of our algorithm, and they are detailed in Section \ref{sec:experments}.

\vspace{5pt}





\vspace{5pt} \noindent \textbf{Printing quality optimization:} It is obvious that mechanical errors could only be diminished instead of totally eliminating, the errors are basically resulted by the re-positioning error during rotations. Due to that the printed objects by support-effective decomposition may still have small seam near the surface positions of cuttings. We notice that there exist many candidate planes in a direction of $\textbf{n}$ having the same values of objective functions, which provides room for optimizing the printing quality. In our algorithm, we first use mesh saliency to obtain a global saliency map $\mathcal{X}(v)$ on vertices of mesh surface and select the best plane from the set of ambiguous candidate planes according to the following equation:
 
 \begin{equation}
     \arg\min_{\textbf{n}_i} \int_{\partial C} \mathcal{X}(v)dv
 \end{equation}
 
\noindent where $C$ is the seam generated by planar cutting. Similarly, our search algorithm is able to easily incorporate other commonly used criteria in the field of additive manufacturing, such as fin and bridge features \cite{luo2012chopper}, part volume \cite{Chen2015dapper}, so on and so forth.
















\subsection{Support structure}
\label{subsec:support}

\begin{figure}
	\centering
    \subfigure[Tree-like supports]{ 
		\includegraphics[width=0.4\linewidth]{fig/figTreeSup.png}
		}
	 \subfigure[Projected supports]{ 	
		\includegraphics[width=0.4\linewidth]{fig/figProjectSup.png}
	    }
		
	\caption{The sparse tree-like support structures and the recursively projected supports generated by Alg. \ref{algRecurProj}.} %
\end{figure}

\begin{algorithm}[t]
\caption{\texttt{Recursive Projection}}\label{algRecurProj}

\LinesNumbered

\KwIn{The decomposed sub-meshes $M$, the corresponding fabrication sequence $S$.}
\KwOut{Support structures $T$}

\STATE Floating points $F_{pnt}\leftarrow\emptyset$.

\For{each mesh $\mathcal{M}_i \in M$ in reversed $S$}{

\STATE Uniformly sample points $P_i$ on $\mathcal{M}_i$ along the printing direction.

\STATE Detect a set of risky points $P_i^r\subseteq P_i$.

\If{$F_{pnt} \neq \emptyset$
}{
\STATE $P_i^r = F_{pnt} \cup P_i^r$.

\STATE $F_{pnt} \leftarrow \emptyset$
}

\STATE Generate sparse tree-like support structures $T_i$.

\STATE $T=T\cup T_i$.

\STATE Add all remaining floating points into $F_{pnt}$.

}

\STATE Return $T$.
\end{algorithm}

Like the fact that we relax the hard-constraint of support-free of \cite{wu2017RoboFDM} into minimizing the area of risky faces as described in $f_{global}$, the scheme of generating support structure is considerately vital while both feasibility and reliability should be guaranteed. To tackle this problem in a tractable way, we propose a new pattern of support structures called \emph{projective supports} in this case which ensures both printability and collision-free requirements.

Since not all models can be fabricated without support structures after a finite number of planar cuttings, we must find a solution to generate as lower as the possible number of support structures to provide enough supports near overhanging regions. The volume decomposition algorithm described before uses a set of planes to construct collision-free spaces for printing specific regions. In the step of generating support structures for our multi-directional printing system, the most important consideration is not introducing unnecessary collisions into such regions (i.e., making additional support structures of a sub-model lie inside the associated space).

The schemes for generating support structures in 3D printing vary from different printing systems. In our work, we focus more on Fused Deposition Modeling (FDM) printing, and there are many works trying to solve the problem of supports generation in FDM. Existing techniques for generating support structures can be categorized into two classes: The first class is a very reliable way to enclose the bottom of the model using a very dense structure, and this method is widely used in commercial software such as Makerbot\textsuperscript{\textregistered} Makeware\textsuperscript{TM}, Ultimaker\textsuperscript{\textregistered} Cura\textsuperscript{TM}. The second class develops the self-supporting property of FDM, and the overhanging regions can be connected if they are close to each other and such sparse patterns of support structures exhibit significant material-savings. Tree-like supports such as clever-support\cite{vanek2014clever}, Autodesk\textsuperscript{\textregistered} Meshmixer\textsuperscript{TM} and Gradientspace\textsuperscript{\textregistered} Cotangent\textsuperscript{TM}, and bridge-like supports \cite{dumas2014bridging} are available for users to select.

In our work, we generate tree-like support structures to provide additional supports for overhanging regions after applying the volume decomposition algorithm. We use the uniformly sampling strategy to detect all of the point overhang, edge overhang and face overhang. The sampling interval is according to the resolution of depositing nozzle. Here we use $2mm$ as an experienced choice. For each sub-mesh $\mathcal{M}_s$ with its associated spatial space $\Omega_s$, an ideal configuration of support structures $\mathcal{C}_s$ should satisfy that $\mathcal{C}_s \subset \Omega_s$ while the amount of $\mathcal{C}_s$ is minimized. We opt to use the method proposed in \cite{vanek2014clever} to generate sparse tree-like support structures because the newly generated nodes of the tree are guaranteed to be inside $\Omega_s$ during the merging procedure so the corresponding connected structures must be inside $\Omega_s$ as well, while other sparse methods have no such guarantee making them unsuitable for our cases. Moreover, the end nodes of supports tend to converge to the closet surface which is considered efficient, and no needs to post-process the converged supports during multi-directional printing.

The procedure of generating sparse tree-like support structures is tackled as the \emph{minimum Steiner tree problem} and a heuristic greedy-based method is adopted to merge a close pair of support structures \cite{vanek2014clever} progressively. Unlike traditional support generation method which finds an intersecting line between the support points until reaching the base of the printing platform, our case has one solid printing platform, and the others are `virtual plane'. Given the decomposed result of our search algorithm, we have to generate the line segment by projecting support structures recursively. The maximal self-supporting angle for sparse tree-like support structures is $30^\circ$. Moreover, considering the stable issue raised by too many branches, we restrict the maximal number of merging smaller than three times to avoid centralized loads. We detail the proposed recursive projection algorithm in Alg. \ref{algRecurProj}.



















==> biography.tex <==
\begin{IEEEbiography}{John Doe}
Biography text here.
\end{IEEEbiography}

\begin{IEEEbiography}{John Doe}
Biography text here.
\end{IEEEbiography}

\begin{IEEEbiography}{John Doe}
Biography text here.
\end{IEEEbiography}

\begin{IEEEbiography}{John Doe}
Biography text here.
\end{IEEEbiography}

\begin{IEEEbiography}{John Doe}
Biography text here.
\end{IEEEbiography}

==> experiments.tex <==
\section{Experimental Results}
\label{sec:experments}

We implement the proposed search algorithms in a C++ program and tested them on a PC with Intel E5-2698 v3 (running at 2.30GHz) and 128GB RAM. The slicing software for conventional FDM is used to create planar slices and tool paths according to the printing directions determined in our algorithm. G-code for AM can be generated from the planned paths and sent to the motion-control module of our system.

We set up two hardware platforms, which have different configurations to navigate the motions of material extrusions, to verify the effectiveness of our algorithm. One is a Cartesion-space-based four-axis multi-directional printer based on an off-the-shelf standard FDM printer. An additional rotating platform is added to achieve multi-directional printing. The other hardware platform is a joint-space-based system named as \emph{RoboFDM}, which is equipped with an industrial robotic arm and a fixed FDM extruder \cite{wu2017RoboFDM}. 

\begin{figure}[t]
\includegraphics[width=.95\linewidth]{fig/figSystemOverview.jpg}
\caption{To fabricate the models of support-effective volume decomposition, we set up two different multi-directional printing systems. (a) The Cartesian-space based printer modified from a customized FDM printer - Ultimaker 2+, with an additional degree-of-freedom to provide the capability of rotating physical platform. (b) The joint-space based system, which consists of an industrial 6-DOF robotic arm and a fused depositing extruder. The most significant difference between our methods and the conventional FDM approaches is that we provide additional degrees of freedom to the physical platform so the build directions can be changed during printing.} 
\label{figSystem}
\end{figure}

\subsection{Cartesian-space-based system}
The hardware setup of four-axis multi-directional printer is developed on top of an FDM Ultimaker 2+ 3D printer with a rotation platform add-in. Inspired by 4-axis CNC machine, a turbine-shaft structured driven by a step motor is set up vertically and fixed in the basement of Ultimaker which will be lifted up together with z-axis movement. Moreover, we design and fabricated an easy-calibrated plastic platform as shown in fig.\ref{figSystem}(a) which can rotate freely to allow $\pm 60^\circ$ rotation collision-free working space. The printing process with this system is as follows: we first slide all cutting model in CURA software which shares same normal direction and lifts up to fulfill the gap between Ultimaker basement and our platform. Then we preprocess generated G-Code to fit the orientation of current pose. During the printing process, we use Arduino chipboard to control the platform to certain rotation degree precisely.  
\subsection{Joint-space-based system}
The hardware setup of the \emph{RoboFDM} system is mainly composed of a UR5 robotic arm, an FDM extruder fixed on a frame and all other control components. To demonstrate the functionality of printing multi-materials, white and black PLA filaments are used. Different regions on a model can be fabricated by using filaments in different colors. The extruder is fixed in our system, and the relative printing direction and position is realized by the inverse pose of the printing platform attached on a 6-axis UR5 robotic arm. The UR5 Robotic arm is used to provide 6-DOF motion during the process of material accumulation. Considering the accuracy of positioning that can be achieved on a UR robotic \cite{Kruit13} and the speed of fabrication, nozzles with 1mm or 2mm holes are employed in our system. Generally, 2mm nozzles are used for quick fabrication, and 1mm nozzles can fabricate models with better surface quality and more geometric details.

The relative position of the nozzle to the base frame of the robotic arm is also significant as it will be a problem if there are many inaccessible positions and orientations in the working envelope defined around the nozzle. The location to place nozzles should be optimized according to the reachability analysis of the robotic arm. 
First of all, we randomly sample the configurations space of UR5's joints and determine the position and orientations of each configuration point in the Euclidean space. Considering the fixed orientation of nozzle, all samples with facing-down frames are excluded. The remained frames are considered reachable samples (see Fig.\ref{figReachability} for example). The working envelope around a nozzle is defined as a bounding box $\mathcal{B}$ centered at the nozzle. The optimal position of a nozzle can then be determined by the exhaustive search to find a place such that the number of frames falling in $\mathcal{B}$ is maximized. 

\begin{figure}[t]
\centering
\includegraphics[width=.455\linewidth]{figOverview}
\includegraphics[width=.53\linewidth]{figReachability}
\caption{The sample frames of reachable positions and orientations used to find a best position to place the nozzle of printing. The density distribution of reachable configurations are shown in color according to the average distance from a sample to its $k$-nearest-neighbors (with $k=10$) -- red means dense and blue represents sparse. Note that, only $10000$ samples are shown here for the visualization purpose and more than 1M samples are employed in our implementation.} \label{figReachability}
\end{figure} 

\begin{figure*}[!t]
\centerline{\includegraphics[width=6in]{fig/holder.jpg}%
\label{fig_first_case}}
\hfil
\caption{The decomposed and printed results fabricated by our system.}
\label{fig_sim}
\end{figure*}

The motion of UR5 is realized by first determining the pose of its end-effector according to a given position and orientation for material accumulation in the Euclidean space. As illustrated in Fig.\ref{figFrames}, there are five different frames in our system including:
\begin{itemize}
\item \emph{B}: Frame of the base link on the robotic arm, which is also set as the origin of the world coordinate system;
\item \emph{E}: Frame of the end-effector with the origin located at the center of the first base plane to print;
\item \emph{P}: Frame for the current part to be printed with the origin located at the center of the current base plane for printing;
\item \emph{O}: Frame at the current position and orientation to accumulate material;
\item \emph{N}: Frame of the FDM extruder with origin at the end of the nozzle.
\end{itemize}
The relationship among these frames can be defined as 
\begin{equation}\label{eqTransformation}
\mathbf{T}_E^B \mathbf{T}_P^E  \mathbf{T}_O^P = \mathbf{T}_N^B,
\end{equation}
where $\mathbf{T}_N^B$ is a constant matrix as the extruder is fixed in our system, $\mathbf{T}_O^P$ is known according to the tool-path represented by G-code, and $\mathbf{T}_P^E$ can be updated during the printing process. With these known transformations, $\mathbf{T}_E^B$ can be obtained by solving Eq.(\ref{eqTransformation}). After determining $\mathbf{T}^B_E$, inverse kinematics is applied to compute a corresponding configuration in the joint space of UR5. The motion between poses is generated by using the \textit{RRT-Connect}  based planning~\cite{Jr00}, with which collision can be avoided. 

\subsection{Results}
We have tested our system by printing a variety of models in a support-free manner. Figure \ref{figSysPipeline} has shown the whole process of printing a support-free bunny model, where supporting structures must be added below the head and at the ears by using conventional 3D printing (see the right of Fig.\ref{figComparison}). Figure \ref{figExperiments} shows our results of decomposition and fabrication on two other models.

At the same time, we also test the mechanical properties of a model fabricated by RoboFDM and compare it with the same model fabricated by conventional 3D printing. As shown in Fig.\ref{figMechTest}, the stiffness of model fabricated by RoboFDM is weaker, which is mainly caused by the weak adhesion of materials at the interface between two regions. On the other aspect, the delamination of layers happens at nearly the same level of loading (i.e., around 1000N).

==> introduction.tex <==
\section{Introduction}\label{sec:introduction}





\IEEEPARstart{T}{he} technology of 3D printing (also named as Additive Manufacturing or AM) appears in the late 1980s. With the rapid development over 30 years, 3D printing devices especially the Fused Deposition Modeling (FDM)-based 3D printers are now available for customers. However, to tackle the limitation of layer-based manufacturing, research has been taken in the aspects of 1) adding more Degree-of-Freedoms (DOFs) into motion and 2) optimizing shape (or direction) of fabrication \cite{Gao2015}. 

\begin{figure}[t]
\centering
\includegraphics[width=.95\linewidth]{fig/figTeaser.png}
\caption{The snowman models fabricated by the traditional FDM printer and our 4-DOF multi-directional printing system: by rotating to different build directions, the support structures can be substantially reduced.} 
\label{figTeaser}
\end{figure}

Layer-based manufacturing is widely used in commercial 3D printing, which however needs to use additional support structures. Specifically, support structure is used to prevent collapse if a layer to be deposited overhanging: the extruder deposits material to accumulate solid object from the bottom layer to the top layer, overhanging regions which are not supported by the layer below would require such structure. Support structure is considered annoying in 3D printing since it has a set of drawbacks, for example, the removal of support structures is not only tedious but also needs professional skills because inappropriate separations may damage the delicate surface of fabricated objects. The need for support structures has inspired researchers in optimizing the generation of support structures, and the generation techniques of support structures below the layers with overhangs can be traced back to 1990s \cite{williams1992three}.  Several approaches have been developed to weaken the disadvantages of support structures by optimizing the topology of support structures \cite{dumas2014bridging,vanek2014clever}, searching an optimal printing direction on a Gaussian sphere by perceptual training and learning strategy \cite{zhang2015perceptual}. A few approaches have been developed to reduce the usage of supporting structure by either model deformation \cite{Hu2015a} or model decomposition \cite{Herholz2015,wei18supportfree, muntoni2018heightblock,Hu2014}.

The problem of decreasing the usage of support structures can be achieved by multi-directional printing. By using the multi-direction printing devices, a 3D model can be rotated to different directions so the included angle between the normal of faces and the build direction can be simultaneously changed. In other words, the needs of support structures can be redistributed by orienting to different build directions. The problem is how to generate a decomposition as well as plan a sequence of rotations to print.

Before diving into the phase of solving the problem, we must have the problem statement first. Given a model $\mathcal{M}$ fabricated layer by layer along a printing direction $\mathbf{d}$ of a base plane $\pi$, borrowing the definitions of maximal self-support angle $\alpha_{max}$ and the self-supported region presented in \cite{Hu2015a}, whether a face $F$ on $\mathcal{M}$ with its normal $\rm \textbf{n}$ is risky or not can be identified by
\begin{equation}
e(F, \pi)=
\begin{cases}
1 & \mathbf{n} \cdot \mathbf{d} + \sin{( \alpha_{max} ) < 0}, \\
0 & \text{otherwise}.
\end{cases}
\end{equation}

\noindent if $e(F,\pi) = 1$ then $F$ is called \textit{risky} face with a printing base $\pi$; otherwise, it is a \textit{safe} face.
It is clear to see that the needs of support structures are firmly related to the printing direction, which provides the possibility to reduce or eliminate support structures by changing the direction during the printing process. A support-effective volume decomposition of an input mesh should consist of two types of outputs: 1) decomposed sub-meshes $M = \{\mathcal{M}_1, \cdots, \mathcal{M}_N\}$ and 2) the collision-free fabrication sequence $S$ of $M$. If not all support structures are abandoned, additional support structures which are suitable for our multi-directional printing should be integrated into decomposed sub-meshes without violating collision-free requirement. 


Our work evolves from a previously published conference paper \cite{wu2017RoboFDM} in which a support-free additive manufacturing system was proposed using a 6-axis robotic arm. Unlike traditional 3D printers whose motion of printing path is executed by an extruder, the RoboFDM system has a fixed extruder and provides a 6-DOF motion to the platform with the help of robotic arm., along with a segmentation and planning algorithm to decompose a given 3D model into multiple support-free regions as well as plan them into a feasible printing sequence without collision. A skeleton-based-analysis coarse decomposition is adopted at the first phase of the algorithm. However, a portion of 3D models in the real world has no accessible skeleton information, which limits broader applications of the proposed system. 

In this paper, we target a more general problem that uses multi-directional printing system to fabricate support-effective models. Support-free is not a hard-constraint anymore, but effective-support has been considered as the primary objective to be optimized, which means a small number of support structures is allowed if they cannot be completely abandoned. We put efforts on designing a search algorithm under the hard-constraint of collision-free while keeping the support-effective objective minimized. To verify the effectiveness of our proposed algorithm, we set up two different testing platforms including a four-axis multi-directional printer based on an off-the-shelf \emph{Ultimaker\textsuperscript{\textregistered} 2+} FDM printer and a six-degrees-of-freedom printing platform based on a 6-axis robotic arm. The experimental results are encouraging that the annoying support structures can be tremendously reduced with the help of additional degrees-of-freedom even with such a minor modification on an off-the-shelf printer, the expense of updating an off-the-shelf printer is estimated as \$200, which is considered affordable. Our paper makes the following contributions:

\noindent
\begin{itemize}
\item We propose a support-effective volume decomposition algorithm for multi-directional 3D printing, manual assembly after decomposition is no longer needed.
\item A region projection method for the generation of support structures is designed for multi-directional 3D printing when support structures cannot be completely abandoned.
\item We design two multi-directional printing systems, one is modified from an off-the-shelf FDM printer with an additional rotation DOF, and the other is based on an industrial robotic arm, to verify the effectiveness of our proposed decomposition algorithm.
\end{itemize}

The remainder of this paper is organized as follows: Section II reviews the related works, Section III introduces our proposed volume decomposition algorithms, Section IV provides some experimental results and comparisons with our previous method, Section V provides some opinions for future works and concludes the whole paper.












